Energy Security and Resilience: Reviewing Concepts and Advancing Planning Perspectives for Transforming Integrated Energy Systems

Recent events, including the pandemic, geopolitical conflicts, supply chain disruptions, and climate change impacts, have exposed the critical need to ensure energy security and resilience in energy systems. We review existing definitions and interrelations between energy security and resilience, conceptualising these terms in the context of energy system transformations. We introduce a classification of disturbances into shock events and slow burn processes to highlight key challenges to energy system resilience. Examples illustrate their distinct impacts on technical, economic, and environmental system performance over time. We compile relevant recourse options across resilience capacity levels and system planning horizons to address these challenges, emphasising actionable strategies for an increasingly integrated energy system. Finally, we propose policy recommendations to integrate shock events and slow burn processes into future energy system planning, enabling forward-looking decision-making and system design to analyse and mitigate potential disruptions.

==> fig/capacity_concept_original.tex <==
\begin{tikzpicture}

% Color definition
\definecolor{fhgreen}{RGB}{23,156,125}
\definecolor{fhblue}{RGB}{0,91,127}
\definecolor{fhgrey}{RGB}{166,187,200}
\definecolor{fhorange}{RGB}{245,130,32}
\definecolor{fhpurple}{RGB}{124,21,77}
\definecolor{lightgrey}{RGB}{196,210,218}

\setstretch{1.0} % line spacing

% Axes
\draw[->] (0,0) -- (7,0) node[midway, below] {\textbf{Time of exposure}}; % x-axis
\draw[->] (0,0) -- (0,7); % y-axis
\node[align=center] at (3.495,-0.7) {\phantom{\textbf{S}}};
% Labels for y-axis
\node[align=center, rotate=90] at (-0.70,3.495) {\textbf{Disturbance intensity}};
\node[align=center, rotate=90] at (-0.25,1.165) {Small};
\node[align=center, rotate=90] at (-0.25,3.495) {Greater};
\node[align=center, rotate=90] at (-0.25,5.825) {Unbearable};

\foreach \x in {2.33,4.66} {
    \draw[dashed, thin, fhgrey] (\x,0) -- (\x,7);
}

\foreach \y in {2.33,4.66} {
    \draw[dashed, thin, fhgrey] (0,\y) -- (7,\y);
}

% Outlines for the quarter circles
\draw[fhblue] (0,0) -- (0:5.8) arc (0:90:5.8) -- cycle;
\draw[fhgreen] (0,0) -- (0:3.5) arc (0:90:3.5) -- cycle;

\node[align=center] at (1.15,1.15) {\textbf{Stability}\\Absorptive\\capacity};
\node[align=center] at (3.3,3.3) {\textbf{Flexibility}\\Adaptive\\capacity};
\node[align=center] at (5.81,5.81) {\textbf{Change}\\Transformative\\capacity};

\end{tikzpicture}

==> nomenclature.tex <==
% \footnotesize

% \nomenclature[A]{$\Gamma, \gamma$}{Set of planning periods, indexed by $\gamma$}
% \nomenclature[A]{$\mathbb{\Gamma}, \gamma$}{Two-dimensional set of investment and operational planning period combinations, indexed by $\gamma = (\gamma^\text{inv},\gamma^\text{op})$}
% \nomenclature[A]{$\mathcal{T_\gamma}, t$}{Set of time steps for $\gamma \in \Gamma$, $\mathcal{T}_\gamma = \{ t_1, \dots, t_T \}$, indexed by $t$}
% \nomenclature[A]{$\mathcal{I}, i$}{Set of nodes, indexed by $i$}
% \nomenclature[A]{$\mathcal{A}^{\text{CH}_4}, a$}{Set of two-dimensional tuples for CH\textsubscript{4} pipelines between nodes (directed arcs), indexed by $a$}
% \nomenclature[A]{$\mathcal{A}^{\text{H}_2}, a$}{Set of two-dimensional tuples for H\textsubscript{2} pipelines between nodes (undirected arcs), indexed by $a$}
% \nomenclature[A]{$\mathcal{S}_i^{\text{CH}_4}, s$}{Set of CH\textsubscript{4} storage facilities at node $i$, indexed by $s$}
% \nomenclature[A]{$\mathcal{S}_i^{\text{H}_2}, s$}{Set of H\textsubscript{2} storage facilities at node $i$, indexed by $s$}
% \nomenclature[A]{$\mathcal{TE}_i^{\text{CH}_4}, te$}{Set of CH\textsubscript{4} terminal facilities at node $i$, indexed by $te$}
% \nomenclature[A]{$\mathcal{TE}_i^{\text{H}_2}, te$}{Set of H\textsubscript{2} terminal facilities at node $i$, indexed by $te$}
% \nomenclature[A]{$NG_i, g$}{Set of natural gas production facilities at node $i$, indexed by $g$}
% \nomenclature[A]{$BH_i$}{Set of blue H\textsubscript{2} production facilities at node $i$, $BH_i \subseteq NG_i$}
% \nomenclature[A]{$GH_i, g$}{Set of green H\textsubscript{2} production facilities at node $i$, indexed by $g$}
% \nomenclature[A]{$SNG_i, g$}{Set of SNG production facilities at node $i$, $SNG_i \subseteq GH_i$, indexed by $g$}
% \nomenclature[A]{$GY_i, g$}{Set of grey H\textsubscript{2} production facilities at node $i$, indexed by $g$}
% \nomenclature[A]{$BIO_i, g$}{Set of biomethane production facilities at node $i$, indexed by $g$}
% \nomenclature[A]{$DOM_i, g$}{Set of domestic hydrogen production facilities at node $i$, indexed by $g$}

% \nomenclature[B]{$RC_g$}{Steam reforming conversion parameter for blue H\textsubscript{2}}
% \nomenclature[B]{$V^{{(\cdot)}}_{g,\gamma}$}{Annual natural gas/green hydrogen and \gls{sng} production volume}
% \nomenclature[B]{$MC_g$}{\gls{sng} methanation conversion factor}
% \nomenclature[B]{$\overline{P}^{\text{CH}_4}_{a,0}$}{Existing CH\textsubscript{4} pipeline capacity}
% \nomenclature[B]{$\overline{SV}^{\text{CH}_4}_{s,0}$}{Existing CH\textsubscript{4} storage capacity}
% \nomenclature[B]{$\overline{TV}^{\text{CH}_4}_{te,0}$}{Existing LNG terminal capacity}
% \nomenclature[B]{$RF_a$}{Effective repurposing factor}
% \nomenclature[B]{$AV_{s,t,\gamma}$}{Time-dependent availability factor}
% \nomenclature[B]{$MIN_{s}$}{Minimal storage level at storage $s$}
% \nomenclature[B]{$\kappa_{s}$}{Storage self-discharge losses between individual time step at storage $s$}
% \nomenclature[B]{$\kappa_{s}^\text{WD}$}{Ratio of maximal withdrawal rate to volume of storage $s$}
% \nomenclature[B]{$\kappa_{s}^\text{IN}$}{Ratio of maximal injection rate to volume of storage $s$}
% \nomenclature[B]{$\lambda_{s}$}{Self-discharge rate of natural gas storages at storage $s$}
% \nomenclature[B]{$\eta^{\text{in}}_{s}$}{Injection losses of natural gas storages at storage $s$}
% \nomenclature[B]{$\eta^{\text{wd}}_{s}$}{Withdrawal losses of natural gas storages at storage $s$}
% \nomenclature[B]{$TLF^{(\cdot)}_{a}$}{Distance-specific losses for CH\textsubscript{4}/H\textsubscript{2} pipelines}
% \nomenclature[B]{$D^{(\cdot)}_{i,t,\gamma}$}{CH\textsubscript{4}/H\textsubscript{2} demand}
% \nomenclature[B]{$G^{(\cdot)}_{g,t,\gamma}$}{Biomethane or domestic H\textsubscript{2} production}
% \nomenclature[B]{$B^{\text{CO}_2}_{\gamma}$}{CO\textsubscript{2} emission budget per period}
% \nomenclature[B]{$EF^{(\cdot)}_{g}$}{CH\textsubscript{4}/blue hydrogen/grey hydrogen/LNG emission factor}
% \nomenclature[B]{$RF_{te}$}{Reforming conversion parameter for LH\textsubscript{2} terminals at terminal $te$}
% \nomenclature[B]{$GR$}{Market growth rate}
% \nomenclature[B]{$\Delta_\gamma$}{Years per planning period}
% \nomenclature[B]{$\Delta_t$}{Years per time step}
% \nomenclature[B]{$PR_{a,\gamma^\text{inv}}$}{Investment restriction for pipelines}
% \nomenclature[B]{$SR_{s,\gamma^\text{inv}}$}{Investment restriction for storage}
% \nomenclature[B]{$C^{(\cdot)}_{a,\gamma}$}{Lifetime Investment/Repurposing/Decommissioning cost parameter for pipelines/storage/terminals}
% \nomenclature[B]{$C^\text{op}_{(\cdot),\gamma}$}{Operational costs parameter for pipelines/storage/terminals}

% \nomenclature[C]{$ng^\text{}_{g,t,\gamma}$}{Natural gas generation}
% \nomenclature[C]{$bh^\text{}_{g,t,\gamma}$}{Blue H\textsubscript{2} production}
% \nomenclature[C]{$ln^\text{}_{g,t,\gamma}$}{\Gls{lng} import}
% \nomenclature[C]{$lh^\text{}_{g,t,\gamma}$}{LH\textsubscript{2} import}
% \nomenclature[C]{$gh^\text{}_{g,t,\gamma}$}{Green H\textsubscript{2} production}
% \nomenclature[C]{$sn^\text{}_{g,t,\gamma}$}{\Gls{sng} production}
% \nomenclature[C]{$gy_{g,t,\gamma}$}{Grey hydrogen production}
% \nomenclature[C]{$p^{{(\cdot)}}_{a=(i,j),t,\gamma} $}{The unidirectional CH\textsubscript{4}/bidirectional H\textsubscript{2} flows from nodes $i \rightarrow j$}
% \nomenclature[C]{$\overline{p}^{{(\cdot)}}_{a,\gamma}$}{Available CH\textsubscript{4}/H\textsubscript{2} pipeline capacity}
% \nomenclature[C]{$\overline{p}^{{(\cdot)}\uparrow}_{a,\gamma}$}{Newly-built CH\textsubscript{4}/H\textsubscript{2} pipeline capacity}
% \nomenclature[C]{$\overline{p}^{{(\cdot)}\downarrow}_{a,\gamma}$}{Decommissioned CH\textsubscript{4}/H\textsubscript{2} pipeline capacity}
% \nomenclature[C]{$\overline{p}^{{(\cdot)}\text{,rep}{(\cdot)}}_{a,\gamma}$}{Repurposed pipeline capacity}
% \nomenclature[C]{$\overline{sv}^{{(\cdot)}}_{s,\gamma}$}{Available CH\textsubscript{4}/H\textsubscript{2} storage capacity}
% \nomenclature[C]{$\overline{sv}^{{(\cdot)}\uparrow}_{s,\gamma}$}{Newly-built CH\textsubscript{4}/H\textsubscript{2} storage capacity}
% \nomenclature[C]{$\overline{sv}^{{(\cdot)}\downarrow}_{s,\gamma}$}{Decommissioned CH\textsubscript{4}/H\textsubscript{2} storage capacity}
% \nomenclature[C]{$\overline{sv}^{{(\cdot)}\text{,rep}{(\cdot)}}_{s,\gamma}$}{Repurposed storage capacity}
% \nomenclature[C]{$\overline{tv}^{{(\cdot)}}_{te,\gamma}$}{Available CH\textsubscript{4}/H\textsubscript{2} terminal capacity}
% \nomenclature[C]{$\overline{tv}^{{(\cdot)}\uparrow}_{te,\gamma}$}{Newly-built CH\textsubscript{4}/H\textsubscript{2} terminal capacity}
% \nomenclature[C]{$\overline{tv}^{{(\cdot)}\downarrow}_{te,\gamma}$}{Decommissioned CH\textsubscript{4}/H\textsubscript{2} terminal capacity}
% \nomenclature[C]{$\overline{tv}^{{(\cdot)}\text{,rep}{(\cdot)}}_{te,\gamma}$}{Repurposed terminal capacity}
% \nomenclature[C]{$p^{{(\cdot)}\text{,wd}}_{s,t,\gamma}$}{CH\textsubscript{4}/H\textsubscript{2} withdrawal volume}
% \nomenclature[C]{$p^{{(\cdot)}\text{,in}}_{s,t,\gamma}$}{CH\textsubscript{4}/H\textsubscript{2} injection volume}
% \nomenclature[C]{$sl_{s,t,\gamma}$}{Storage level}
% \nomenclature[C]{$gf_{i,t,\gamma}$}{Natural gas flare}

% \printnomenclature
